CSSTs: A Dynamic Data Structure for Partial Orders in Concurrent Execution Analysis

Dynamic analyses are a standard approach to analyzing and testing concurrent programs. Such techniques observe program traces and analyze them to infer the presence or absence of bugs. At its core, each analysis maintains a partial order $P$ that represents order dependencies between events of the analyzed trace $\sigma$. Naturally, the scalability of the analysis largely depends on how efficiently it maintains $P$. The standard data structure for this task has thus far been vector clocks. These, however, are slow for analyses that follow a non-streaming style, costing $O(n)$ for inserting (and propagating) each new ordering in $P$, where $n$ is the size of $\sigma$, while they cannot handle the deletion of existing orderings. In this paper we develop collective sparse segment trees (CSSTs), a simple but elegant data structure for generically maintaining a partial order $P$. CSSTs thrive when the width $k$ of $P$ is much smaller than the size $n$ of its domain, allowing inserting, deleting, and querying for orderings in $P$ to run in $O(logn)$ time. For a concurrent trace, $k$ is bounded by the number of its threads, and is normally orders of magnitude smaller than its size $n$, making CSSTs fitting for this setting. Our experimental results confirm that CSSTs are the best data structure currently to handle a range of dynamic analyses from existing literature.

==> material/figures/scalability_bk.tex <==
\begin{figure*}[!h]
\def\height{4cm}
\def\width{5.2cm}
\pgfplotsset{compat=newest}
\scalebox{0.9}{%
\begin{tikzpicture}
\begin{groupplot}[
group style={group size= 4 by 2, vertical sep=1.5cm} , 
every x tick scale label/.style={at={(1,0)},xshift=1pt,anchor=south west,inner sep=0pt},
legend to name=named,
legend columns=-1
]
\nextgroupplot[
inner sep=2pt,
width=\width,
height=\height,
ylabel={Time (s)},
ylabel near ticks,
xlabel={$\numEvents$},
grid=both,
clip=false,
axis lines*=left,
title={Insert, $\numThreads=10$},
ymin={0},
xtick distance=0.25e6,
ytick distance=0.25e-4,
]

\addplot table[x=x, y=cssts, col sep=comma]{scalability_sts_insert_k=10_r=10000_i=20n.csv};\label{plots:curve_cssts}
\addplot table[x=x, y=sts, col sep=comma]{scalability_sts_insert_k=10_r=10000_i=20n.csv};\label{plots:curve_vcs}
\coordinate (c1) at (rel axis cs:0,1);



\nextgroupplot[
inner sep=2pt,
width=\width,
height=\height,
ylabel={Time (s)},
ylabel near ticks,
xlabel={$\numEvents$},
grid=both,
clip=false,
axis lines*=left,
title={Insert, $\numThreads=20$},
xtick={0.25e6,0.5e6,0.75e6,1e6},
ymin={0},
xtick distance=0.25e6,
ytick distance=1e-4,
]

\addplot table[x=x, y=cssts, col sep=comma]{scalability_sts_insert_k=20_r=10000_i=20n.csv};
\addplot table[x=x, y=sts, col sep=comma]{scalability_sts_insert_k=20_r=10000_i=20n.csv};




\nextgroupplot[
inner sep=2pt,
width=\width,
height=\height,
ylabel={Time (s)},
ylabel near ticks,
xlabel={$\numEvents$},
grid=both,
clip=false,
axis lines*=left,
title={Query, $\numThreads=10$},
ymin={0},
xtick distance=0.25e6,
ytick distance=1e-6,
]

\addplot table[x=x, y=cssts, col sep=comma]{scalability_sts_query_k=10_r=10000_i=20n.csv};
\addplot table[x=x, y=sts, col sep=comma]{scalability_sts_query_k=10_r=10000_i=20n.csv};




\nextgroupplot[
inner sep=2pt,
width=\width,
height=\height,
ylabel={Time (s)},
ylabel near ticks,
xlabel={$\numEvents$},
grid=both,
clip=false,
axis lines*=left,
title={Query, $\numThreads=20$},
ymin={0},
xtick distance=0.25e6,
ytick distance=2e-6,
]

\addplot table[x=x, y=cssts, col sep=comma]{scalability_sts_query_k=20_r=10000_i=20n.csv};
\addplot table[x=x, y=sts, col sep=comma]{scalability_sts_query_k=20_r=10000_i=20n.csv};
\coordinate (c2) at (rel axis cs:1,1);





%%%%%%%%%% Replace with VCs


\nextgroupplot[
inner sep=2pt,
width=\width,
height=\height,
ylabel={Time (s)},
ylabel near ticks,
xlabel={$\numEvents$},
grid=both,
clip=false,
axis lines*=left,
title={Insert, $\numThreads=10$},
ymin={0},
xtick distance=0.25e6,
ytick distance=0.25e-4,
]

\addplot table[x=x, y=cssts, col sep=comma]{scalability_sts_insert_k=10_r=10000_i=20n.csv};
\addplot[mark=diamond*, mark size=3pt,color=olive] table[x=x, y=sts, col sep=comma]{scalability_sts_insert_k=10_r=10000_i=20n.csv};\label{plots:curve_sts}



\nextgroupplot[
inner sep=2pt,
width=\width,
height=\height,
ylabel={Time (s)},
ylabel near ticks,
xlabel={$\numEvents$},
grid=both,
clip=false,
axis lines*=left,
title={Insert, $\numThreads=20$},
xtick={0.25e6,0.5e6,0.75e6,1e6},
ymin={0},
xtick distance=0.25e6,
ytick distance=1e-4,
]

\addplot table[x=x, y=cssts, col sep=comma]{scalability_sts_insert_k=20_r=10000_i=20n.csv};
\addplot[mark=diamond*, mark size=3pt,color=olive] table[x=x, y=sts, col sep=comma]{scalability_sts_insert_k=20_r=10000_i=20n.csv};




\nextgroupplot[
inner sep=2pt,
width=\width,
height=\height,
ylabel={Time (s)},
ylabel near ticks,
xlabel={$\numEvents$},
grid=both,
clip=false,
axis lines*=left,
title={Query, $\numThreads=10$},
ymin={0},
xtick distance=0.25e6,
ytick distance=1e-6,
]

\addplot table[x=x, y=cssts, col sep=comma]{scalability_sts_query_k=10_r=10000_i=20n.csv};
\addplot[mark=diamond*, mark size=3pt,color=olive] table[x=x, y=sts, col sep=comma]{scalability_sts_query_k=10_r=10000_i=20n.csv};




\nextgroupplot[
inner sep=2pt,
width=\width,
height=\height,
ylabel={Time (s)},
ylabel near ticks,
xlabel={$\numEvents$},
grid=both,
clip=false,
axis lines*=left,
title={Query, $\numThreads=20$},
ymin={0},
xtick distance=0.25e6,
ytick distance=2e-6,
]

\addplot table[x=x, y=cssts, col sep=comma]{scalability_sts_query_k=20_r=10000_i=20n.csv};
\addplot[mark=diamond*, mark size=3pt,color=olive] table[x=x, y=sts, col sep=comma]{scalability_sts_query_k=20_r=10000_i=20n.csv};


\legend{Line 1, Line 2}
\end{groupplot}
      
\end{tikzpicture}

\ref{named}

}%
\caption{
\Andreas{
Caption
}
}
\label{fig:scalability}
\end{figure*}







%\begin{figure*}[!h]
%\def\height{5cm}
%\def\width{7cm}
%\begin{subfigure}{0.475\textwidth}
%\begin{tikzpicture}
%\begin{axis}[
%inner sep=2pt,
%width=\width,
%height=\height,
%ylabel={Time (s)},
%ylabel near ticks,
%xlabel={$\numEvents$},
%grid=both,
%clip=false,
%axis lines*=left,
%title={Insert},
%]
%
%\addplot table[x=x, y=cssts, col sep=comma]{scalability_sts_insert_k=10_r=10000_i=20n.csv};
%\addplot table[x=x, y=sts, col sep=comma]{scalability_sts_insert_k=10_r=10000_i=20n.csv};
%
%\legend{\small $\ds$, $\naiveds$}
%\end{axis}
%\end{tikzpicture}
%\end{subfigure}
%\caption{
%\Andreas{
%Caption
%}
%}
%\label{fig:scalability}
%\end{figure*}
%
%
%
%
%


==> sections/ds-incremental-beginning.tex <==
\subsection{Fully Dynamic $\ds$}\label{sec:ds-full}

We now present fully dynamic $\ds$.
Their properties are stated in the following theorem.


\begin{restatable}{theorem}{thmdsdynamic}\label{thm:ds_dynamic}
Consider a chain DAG $G$ of $\numEvents$ nodes and $\numThreads$ chains.
$\ds$ correctly maintain $G$ under dynamic updates, costing $O(\log n)$ time per update and $O(\numThreads^3 m)$ time per query,
where $m=\min(\log n, d)$, and $d$ is the cross-chain density of $G$.
\end{restatable}

Compared to \cref{thm:ds_incremental}, \cref{thm:ds_dynamic} trades the cost dependency on the number of threads from updates to queries, while also increasing it by a factor $\numThreads$.
Moreover, the upper bound on updates is now $O(\log n)$, i.e., independent of $d$.
For analyses that maintain partial orders only incrementally, both versions of $\ds$ can be used,
but we expect \cref{thm:ds_incremental} to be more performant due to the lower dependency on $\numThreads$, and especially when queries outnumber updates.
Fully dynamic analyses are handled by the $\ds$ of \cref{thm:ds_dynamic}.


\myparagraph{Intuition}
The support of both insert and delete operations is based on two key ideas.
First, instead of keeping $\ds$ transitively-closed across chains, we only store direct edges in them,
as described in \cref{subsec:dynamic-suffix-minima}.
This way, an edge deletion does not have to rollback any transitive orderings that were going through it,
which would be challenging to perform efficiently.
Instead, transitive orderings are now found during queries, by performing a forward/backward search from the source node.

Second, since each entry $\dsarray{t_1}{t_2}[j_1]$ stores the highest immediate successor of $\graphnode{t_1}{j_1}$ in chain $j_2$,
when this edge is deleted, we have to efficiently recover the next highest successor.
We achieve this by maintaining all current successors of $\graphnode{t_1}{j_1}$ to chain $t_2$ in a min heap $\edgeheap_{t_1}^{t_2}[j_1]$,
and $\dsarray{t_1}{t_2}[j_1]$ always stores the top of the heap.


\myparagraph{Fully dynamic $\ds$}
The pseudocode for fully dynamic $\ds$ is shown in \cref{algo:ds-full-interface}, following the description above.
The functions $\FunctionInsertEdge$ and $\FunctionDeleteEdge$ manipulate the min-heaps $\edgeheap_{t_1}^{t_2}[j_1]$, storing edges that go from $\graphnode{t_1}{j_1}$ to chain $t_2$.
The function  $\FunctionQuery$ is implemented via a $\suc$ query, as in \cref{algo:ds-inc-interface}.
In turn, $\suc$ is the most involved function, as it performs a forward traversal from $\graphnode{t_1}{j_1}$ to discover transitive reachability information.
This is performed by repeated $\mn$ queries in the suffix minima arrays $\dsarray{t'_1}{t'_2}$, which attempt to find the earliest successor of thread $t'_2$ that can be reached in one step by the currently highest node of $t'_1$ already reachable from the source node $\graphnode{t_1}{j_1}$.
The crucial property of this computation is that, using suffix minima queries,  it completes in $O(\numThreads^3)$ steps, as opposed to $O(\numEvents^2)$ steps which is the standard complexity of a graph traversal, and thus remains efficient and within the targeted bounds of \cref{thm:ds_dynamic}.


\input{material/algorithms/opt-ds/interface-full}

\input{material/examples/ds-full}


\myparagraph{Analysis}
We now state the properties of fully dynamic $\ds$.
First,  since the arrays $\dsarray{t_1}{t_2}$ only store direct edges, a sparsity property analogous to \cref{lem:ds-inc-sparsity} follows directly.

\begin{restatable}[Sparsity]{lemma}{lemdssparsity}\label{lem:ds-sparsity}
Let $d$ be the cross-chain density of $G$.
Then the density of each array $\dsarray{t_1}{t_2}$ is bounded by $d$.
\end{restatable}

It is straightforward to see that, using the min-heaps $\edgeheap_{t_1}^{t_2}[j_1]$,  fully dynamic $\ds$ maintain the following invariant,
which concerns the correctness of the updates.

\begin{restatable}[Invariant]{lemma}{lemdsinvariant}\label{lem:ds-invariant}
For every distinct $t_1, t_2\in [\numThreads]$,
$\dsarray{t_1}{t_2}[j_1] = \min(\{j_2\in [\numEvents].~\graphnode{t_1}{j_1}\to \graphnode{t_2}{j_2}\})$.
\end{restatable}

Since every node has $\leq \numEvents$ successors, each heap operation clearly runs in $O(\log n)$ time, which is the complexity of updates.
The following lemma implies the correctness of queries, while, together with \cref{lem:ds-sparsity}, also yields the complexity of queries, thus concluding \cref{thm:ds_dynamic}.

\begin{restatable}{lemma}{lemdscomplexitysuc}\label{lem:ds-complexity-suc}
For every $i\in[\numThreads]$, the $i$-th iteration of the do-while loop in \cref{line:algo_ds_do},
there are $i$ threads $t$ for which $\closure_{t_1}^{t}[j_1]=\min(\{j\in [\numEvents].~\graphnode{t}{j_1}\to \graphnode{t}{j}\})$.
\end{restatable}



==> sections/ds-incremental-main.tex <==

\input{sections/3-ds/4-ds}


==> sections/experiments-random_testing.tex <==





==> sections/experiments-velodrome.tex <==
%!TEX root = ../../main.tex

\subsection{Atomicity Violation Detection}

Velodrome~\cite{Flanagan-2008}.
Velodrome internally utilizes explicit graphs for handling reachability.
We implemented $\ds$ and $\vc$ inside Velodrome~\cite{Flanagan-2008}.


\input{material/tables/velodrome-result.tex}

==> sections/prelim-illustrate.tex <==
%!TEX root = ../../main.tex

% Illustrate the definitions in an example.

%\input{material/examples/def}


\begin{example}
	\label{prelim-defs}
%	We illustrate the presented definitions with concrete examples.
%\Andreas{@Hunkar: Also write what the cross-chain density of $G$ is.}
	Consider the execution $\tr$ and the partial order $\partialord{\tr}$ shown in $\cref{fig:motivating-1}$.
	We have $\events{\tr}=\set{e_1, \ldots, e_n}$ and $\threads{\tr}=\set{0, 1, 2}$.
	%In this setting, the meta information stored in the events correspond to the type of operation performed. 
	%read events store the write event that they are reading from as meta information.
	The events $e_1$ and $e_2$ are represented as $\tuple{0, 0, \set{\wt(x, 1)}}$ and $\tuple{0, 1, \set{\rd(y, 5)}}$, respectively.
	%Observe that $\metaof{e_1}$ is empty and $\metaof{e_2}=e_3$ where $\rf{\tr}(e_2) = e_3$.
	We have $e_5 \partialord{\tr} e_n$ and $e_4 \partialord{\tr} e_3$ and $e_1 \tho{\tr} e_2$ and $e_7 \tho{\tr} e_n$.
	On the other hand $e_1 \unord{\tr}{P} e_4$ and $e_1 \unord{\tr}{P} e_7$.
	The cross-chain density of $G$ is $2$ due to $\sub{G}{1}{2}$, which has the maximum number of cross-edges across all sub-graphs.
	Some queries on $G$ are
	\begin{compactitem}
		\item $\reachable(e_1, e_5) = False$, $\reachable(e_4, e_3) = True$
		\item $\suc(e_4, t_3) = e_7, \suc(e_5, t_1) = e_2$
		\item $\pred(e_3, t_2) = e_6$,  $\pred(e_3, t_3) = e_n$
	\end{compactitem}
	%Examples of events unordered by $\partialord{\tr}$ are $e_1 \unord{\tr}{P} e_3$ and $e_1 \unord{\tr}{P} e_6$.
	%The width of the constructed partial order $\width(\partialord{\tr}) = 3$.
	%The meta information $\metaof(e)$ can be the operation performed by $e$. 
	%For instance be read/write operation on a memory location $x$, denoted by $\rd{(x)}$ and $\wt{(x)}$, or acquire/release of a lock $l$, denoted by $\acq{(l)}$ and $\rel{(l)}$. 
	%Consider now the \cref{fig:defs}.
	%Observe that the DAG $G$ in \cref{subfig:defs-dag} has $\width(G)=3$.

	%The arrays representing the edges across chains in the sparse representation of $G$ are shown in \cref{fig:defs}.
	%Certain example queries on this DAG are as follows.
	%\begin{itemize}
	%	\item $\reachable(\graphnode{t_1}{1}, \graphnode{t_3}{2}) = True$
	%	\item $\reachable(\graphnode{t_1}{3}, \graphnode{t_3}{2}) = False$
	%	\item $\suc(\graphnode{t_1}{0}, t_2) = \graphnode{t_2}{0}$
	%	\item $\suc(\graphnode{t_1}{1}, i_2) = \suc(\graphnode{t_1}{2}, i_2) = \graphnode{2}{1}$
	%	\item $\pred(\graphnode{t_2}{3}, i_1) = \graphnode{t_1}{3}$
	%	\item $\pred(\graphnode{t_2}{1}, i_1) = \pred(\graphnode{t_3}{3}, i_1) = \graphnode{1}{2}$
	%\end{itemize}
\end{example}

==> sections/related_work-beginning.tex <==
%!TEX root = main.tex

\section{Conclusion}

We have introduced $\ds$, a simple yet elegant data structure for the fully-dynamic maintenance of partial orders with small width $\numThreads$, supporting a plethora of dynamic analyses for concurrency.
$\ds$ allow for inserting and deleting new orderings, as well as querying whether two events are ordered, each in time $O(\log \numEvents)$  when $\numThreads=O(1)$.
Our experimental results indicate that $\ds$ are an efficient, drop-in replacement of existing approaches to maintaining partial orders in various application domains of recent literature.
Our aim is thus for $\ds$ to become a standard reference for driving future scalable dynamic analyses.
